Risk aggregation with empirical margins: Latin hypercubes, empirical copulas, and convergence of sum distributions

This paper studies convergence properties of multivariate distributions constructed by endowing empirical margins with a copula. This setting includes Latin Hypercube Sampling with dependence, also known as the Iman--Conover method. The primary question addressed here is the convergence of the component sum, which is relevant to risk aggregation in insurance and finance. This paper shows that a CLT for the aggregated risk distribution is not available, so that the underlying mathematical problem goes beyond classic functional CLTs for empirical copulas. This issue is relevant to Monte-Carlo based risk aggregation in all multivariate models generated by plugging empirical margins into a copula. Instead of a functional CLT, this paper establishes strong uniform consistency of the estimated sum distribution function and provides a sufficient criterion for the convergence rate $O(n^{-1/2})$ in probability. These convergence results hold for all copulas with bounded densities. Examples with unbounded densities include bivariate Clayton and Gauss copulas. The convergence results are not specific to the component sum and hold also for any other componentwise non-decreasing aggregation function. On the other hand, convergence of estimates for the joint distribution is much easier to prove, including CLTs. Beyond Iman--Conover estimates, the results of this paper apply to multivariate distributions obtained by plugging empirical margins into an exact copula or by plugging exact margins into an empirical copula.

==> AuxFiles/AMS_classifications.tex <==
\par
%\vspace{0.5em}
\noindent%\vspace{1em}
AMS 2000 subject classification:

62G09; %Resampling methods
62G20; %Asymptotic properties
62G30; %Order statistics; empirical distribution functions
62P05; %Applications to actuarial sciences and financial mathematics
62H99  %62Hxx: Multivariate analysis None of the above, but in this section


% 60Exx Distribution theory [See also 62Exx, 62Hxx]
%       60E05 Distributions: general theory
%	60E07 Infinitely divisible distributions; stable distributions
%	60E10 Characteristic functions; other transforms
%	60E15 Inequalities; stochastic orderings
%	60E99 None of the above, but in this section
% 62Gxx: Nonparametric inference
%     * 62G05 Estimation
%     * 62G07 Density estimation
%     * 62G08 Nonparametric regression
%     * 62G09 Resampling methods
%     * 62G10 Hypothesis testing
%     * 62G15 Tolerance and confidence regions
%     * 62G20 Asymptotic properties
%     * 62G30 Order statistics; empirical distribution functions
%     * 62G32 Statistics of extreme values; tail inference
%     * 62G35 Robustness
%     * 62G99 None of the above, but in this section
% 62Pxx: Applications
% [See also 90-xx, 91-xx, 92-xx]
%     * 62P05 Applications to actuarial sciences and financial mathematics
%     * 62P10 Applications to biology and medical sciences
%     * 62P12 Applications to environmental and related topics
%     * 62P15 Applications to psychology
%     * 62P20 Applications to economics [See also 91Bxx]
%     * 62P25 Applications to social sciences
%     * 62P30 Applications in engineering and industry
%     * 62P35 Applications to physics
%     * 62P99 None of the above, but in this section
% 62Hxx: Multivariate analysis
% [See also 60Exx]
%     * 62H05 Characterization and structure theory
%     * 62H10 Distribution of statistics
%     * 62H11 Directional data; spatial statistics
%     * 62H12 Estimation
%     * 62H15 Hypothesis testing
%     * 62H17 Contingency tables
%     * 62H20 Measures of association (correlation, canonical correlation, etc.)
%     * 62H25 Factor analysis and principal components; correspondence analysis
%     * 62H30 Classification and discrimination; cluster analysis [See also 68T10]
%     * 62H35 Image analysis
%     * 62H99 None of the above, but in this section
%
%

%
% I could not find this in the manual:
%
% \noindent\textbf{JEL classification}\,\ C13 $\cdot$ C14 $\cdot$ G11
%
% JEL classification (C = Mathematics / Quantitative methods)
%C1 - Econometric and Statistical Methods: General
%       C10 - General
%       C11 - Bayesian Analysis
%       C12 - Hypothesis Testing
%       C13 - Estimation
%       C14 - Semiparametric and Nonparametric Methods
%       C15 - Simulation Methods
%       C16 - Specific Distributions
%       C19 - Other
%
% C4 - Econometric and Statistical Methods: Special Topics
%       C40 - General
%       C41 - Duration Analysis
%       C43 - Index Numbers and Aggregation
%       C44 - Statistical Decision Theory; Operations Research
%       C45 - Neural Networks and Related Topics
%       C46 - Specific Distributions; Specific Statistics
%       C49 - Other 
% G - Financial Economics
% G0 - General
%       G00 - General
%       G01 - Financial Crises
% G1 - General Financial Markets
%       G10 - General
%       G11 - Portfolio Choice; Investment Decisions
%       G12 - Asset Pricing; Trading volume; Bond Interest Rates
%       G13 - Contingent Pricing; Futures Pricing
%       G14 - Information and Market Efficiency; Event Studies
%       G15 - International Financial Markets
%       G17 - Financial Forecasting
%       G18 - Government Policy and Regulation
%       G19 - Other
% G3 - Corporate Finance and Governance
%       G30 - General
%       G31 - Capital Budgeting; Fixed Investment and Inventory Studies
%       G32 - Financing Policy; Financial Risk and Risk Management; Capital and Ownership Structure
%       G33 - Bankruptcy; Liquidation
%       G34 - Mergers; Acquisitions; Restructuring; Corporate Governance
%       G35 - Payout Policy
%       G38 - Government Policy and Regulation
%       G39 - Other 


==> AuxFiles/zzz_print_custom_commands.tex <==
\input{mydefs-journal}
\input{mycommands}
%

\addtolength{\textheight}{6cm}


\voffset-1cm

\begin{document}

$\begin{array}{l} \verb+\abs+   \text{\quad---\quad}  \abs{\displaystyle\sum_0^\infty x^3}
\\ \verb+\absfl+  \text{\quad---\quad}  \absfl{\displaystyle\sum_0^\infty x^3}
\\ \verb+\Acal+  \text{\quad---\quad}   \Acal
\\ \verb+\alphaast+  \text{\quad---\quad}  \alphaast
\\ \verb+\alphadeltaeps+  \text{\quad---\quad}  \alphadeltaeps
\\ \verb+\alphahat+  \text{\quad---\quad}  \alphahat
\\ \verb+\alphahatHill+  \text{\quad---\quad}  \alphahatHill
\\ \verb+\alphai+  \text{\quad---\quad}  \alphai
\\ \verb+\alphaiplusone+  \text{\quad---\quad}  \alphaiplusone
\\ \verb+\alpham+  \text{\quad---\quad}  \alpham
\\ \verb+\alphan+  \text{\quad---\quad}  \alphan
\\ \verb+\alphanstr+  \text{\quad---\quad}  \alphanstr
\\ \verb+\alphanstrstr+  \text{\quad---\quad}  \alphanstrstr
\\ \verb+\alphaone+  \text{\quad---\quad}  \alphaone
\\ \verb+\alphatwo+  \text{\quad---\quad}  \alphatwo
\\ \verb+\alphapr+  \text{\quad---\quad}  \alphapr
\\ \verb+\alphaX+  \text{\quad---\quad}  \alphaX
\\ \verb+\alphaY+  \text{\quad---\quad}  \alphaY
\\ \verb+\Aei+  \text{\quad---\quad}  \Aei
\\ \verb+\Aej+  \text{\quad---\quad}  \Aej
\\ \verb+\Anorm+  \text{\quad---\quad}  \Anorm
\\ \verb+\Aone+  \text{\quad---\quad}  \Aone
\\ \verb+\argmax+  \text{\quad---\quad}  \argmax
\\ \verb+\argmin+  \text{\quad---\quad}  \argmin
\\ \verb+\asconv+  \text{\quad---\quad}  \asconv
\\ \verb+\asoutconv+  \text{\quad---\quad}  \asoutconv
\\ \verb+\At+  \text{\quad---\quad}  \At
\\ \verb+\AX+  \text{\quad---\quad}  \AX
\\ \verb+\Axione+  \text{\quad---\quad}  \Axione
\\ \verb+\Axioptone+  \text{\quad---\quad}  \Axioptone
\\ \verb+\Axihatoptone+  \text{\quad---\quad}  \Axihatoptone
\\ \verb+\Axit+  \text{\quad---\quad}  \Axit
\\ \verb+\axiX+  \text{\quad---\quad}  \axiX
\\ \verb+\axiY+  \text{\quad---\quad}  \axiY
\\ \verb+\AY+  \text{\quad---\quad}  \AY
\end{array}$


$\begin{array}{l}
  \verb+\Bdelta+  \text{\quad---\quad}  \Bdelta
\\ \verb+\bH+  \text{\quad---\quad}  \bH
\\ \verb+\BLone+  \text{\quad---\quad}  \BLone
\\ \verb+\bnd+  \text{\quad---\quad}  \bnd (= \verb+\partial+)
\\ \verb+\Borel+  \text{\quad---\quad}  \Borel
\\ \verb+\Bxidelta+  \text{\quad---\quad}  \Bxidelta
\end{array}$


$\begin{array}{l}
   \verb+\cadlag+  \text{\quad---\quad}  \text{\cadlag\cadlag,text}
\\ \verb+\Ccal+  \text{\quad---\quad}  \Ccal
\\ \verb+\Ccalb+  \text{\quad---\quad}  \Ccalb
\\ \verb+\Cervonenkis+  \text{\quad---\quad}  \text{\Cervonenkis\Cervonenkis,text}
\\ \verb+\Cii+  \text{\quad---\quad}  \Cii
\\ \verb+\Cij+  \text{\quad---\quad}  \Cij
\\ \verb+\Ctilde+  \text{\quad---\quad}  \Ctilde
\\ \verb+\Ctildeii+  \text{\quad---\quad}  \Ctildeii
\\ \verb+\Ctildeij+  \text{\quad---\quad}  \Ctildeij
\end{array}$


$\begin{array}{l}
\verb+X\compd+  \text{\quad---\quad}  XXX\compd, yyy\compd
\\ \verb+X\compdminusone+  \text{\quad---\quad}  XXX\compdminusone, ZZZ\compdminusone
\\ \verb+x\compi+  \text{\quad---\quad}  XXX\compi
\\ \verb+x\compid+  \text{\quad---\quad}  XXX\compid
\\ \verb+x\compim+  \text{\quad---\quad}  XXX\compim
\\ \verb+x\compione+  \text{\quad---\quad}  XXX\compione
\\ \verb+x\compj+  \text{\quad---\quad}  XXX\compj
\\ \verb+x\compone+  \text{\quad---\quad}  XXX\compone
%{\compn+  \text{\quad---\quad}  ^{(n)}}
\\ \verb+x\comptwo+  \text{\quad---\quad}  XXX\comptwo
\end{array}$


$\begin{array}{l}
\verb+\cubr{\displaystyle\sum x}+  \text{\quad---\quad}  \cubr{\displaystyle\sum x}
\\ \verb+\cubrfl{\displaystyle\sum x}+  \text{\quad---\quad}  \cubrfl{\displaystyle\sum x}
\\ \verb+\CX+  \text{\quad---\quad}  \CX
\\ \verb+\cxialpha+  \text{\quad---\quad}  \cxialpha
\\ \verb+\cxionealpha+  \text{\quad---\quad}  \cxionealpha
\\ \verb+\cxipalpha+  \text{\quad---\quad}  \cxipalpha
\\ \verb+\CY+  \text{\quad---\quad}  \CY
\end{array}$


$\begin{array}{l}
   \verb+\Deltai+  \text{\quad---\quad}  \Deltai
\\ \verb+\deltaij+  \text{\quad---\quad}  \deltaij
\\ \verb+\deriv{.}+  \text{\quad---\quad}  \deriv{X}, \deriv{Y}
\\ \verb+\derivsec{.}+  \text{\quad---\quad}  \derivsec{X}, \derivsec{Y}
\\ \verb+\Dii+  \text{\quad---\quad}  \Dii
\\ \verb+\Dirac{x}+  \text{\quad---\quad}  \Dirac{X}
\\ \verb+\dirprodionek+  \text{\quad---\quad} \dirprodionek
\\ \verb+\disteq+  \text{\quad---\quad}  \disteq
\\ \verb+\Dbb+  \text{\quad---\quad}  \Dbb
\\ \verb+\dBLone+  \text{\quad---\quad}  \dBLone
\\ \verb+\Dcal+  \text{\quad---\quad}  \Dcal
\\ \verb+\dinf+  \text{\quad---\quad}  \dinf
\\ \verb+\dm+  \text{\quad---\quad} \dm
\\ \verb+\done+  \text{\quad---\quad} \done
\\ \verb+\Done+  \text{\quad---\quad} \Done
\\ \verb+\Donetwo+  \text{\quad---\quad}  \Donetwo
\\ \verb+\downto+  \text{\quad---\quad}  \downto
\\ \verb+\downtozer+  \text{\quad---\quad}  \downtozer
\\ \verb+\Dtwo+  \text{\quad---\quad}  \Dtwo
\end{array}$


$\begin{array}{l}\verb+\E+  \text{\quad---\quad}  \E
\\ \verb+\Ecal+  \text{\quad---\quad}  \Ecal
\\ \verb+\Ecalzer+  \text{\quad---\quad}  \Ecalzer
\\ \verb+\Eout+  \text{\quad---\quad}  \Eout
\\ \verb+\East+  \text{\quad---\quad}  \East
\\ \verb+\Ebb+  \text{\quad---\quad}  \Ebb
\\ \verb+\ei+  \text{\quad---\quad}  ei
\\ \verb+\ej+  \text{\quad---\quad}  ej
\\ \verb+\enquote{text}+  \text{\quad---\quad}  \text{\enquote{text}}
\\ \verb+\eps+  \text{\quad---\quad}  \eps
\\ \verb+\ES+  \text{\quad---\quad}  \textit{ ES $\ES$ ES} \text{\quad ((mittleres ES))}
%{\ESlam+  \text{\quad---\quad}  \ES_\lambda}
\\ \verb+\ESoneminuslam+  \text{\quad---\quad}  \ESoneminuslam
\end{array}$


$\begin{array}{l}\verb+\Fab+  \text{\quad---\quad}  \Fab
\\ \verb+\fast+  \text{\quad---\quad}  \fast
\\ \verb+\Fbar+  \text{\quad---\quad}  \Fbar
\\ \verb+\FbarXcompone+  \text{\quad---\quad}  \FbarXcompone
\\ \verb+\FbarYcompone+  \text{\quad---\quad}  \FbarYcompone
\\ \verb+\FbarxitrX+  \text{\quad---\quad}  \FbarxitrX
\\ \verb+\FbarxitrY+  \text{\quad---\quad}  \FbarxitrY
\end{array}$


$\begin{array}{l}\verb+\Fbb+  \text{\quad---\quad}  \Fbb
\\ \verb+\Fbbk+  \text{\quad---\quad}  \Fbbk
\\ \verb+\Fcal+  \text{\quad---\quad}  \Fcal
\\ \verb+\Fcalalphaast+  \text{\quad---\quad}  \Fcalalphaast
\\ \verb+\FcalalphaastH+  \text{\quad---\quad}  \FcalalphaastH
\\ \verb+\Fcalast+  \text{\quad---\quad}  \Fcalast
\\ \verb+\Fcalastdelta+  \text{\quad---\quad}  \Fcalastdelta
\\ \verb+\FcalH+  \text{\quad---\quad}  \FcalH
\\ \verb+\FcalHalpha+  \text{\quad---\quad}  \FcalHalpha
\\ \verb+\FcalHI+  \text{\quad---\quad}  \FcalH
\\ \verb+\FcalHK+  \text{\quad---\quad}  \FcalHK
\\ \verb+\FcalHoneK+  \text{\quad---\quad}  \FcalHoneK
\\ \verb+\Fcaltwoalphaast+  \text{\quad---\quad}  \Fcaltwoalphaast
\\ \verb+\FcalSimpd+  \text{\quad---\quad}  \FcalSimpd
\\ \verb+\FcalSimpdK+  \text{\quad---\quad}  \FcalSimpdK
\\ \verb+\Fcaltilde+  \text{\quad---\quad}  \Fcaltilde
\\ \verb+\FcaltildeHalpha+  \text{\quad---\quad}  \FcaltildeHalpha
\\ \verb+\FR+  \text{\quad---\quad}  \FR
\\ \verb+\fR+  \text{\quad---\quad}  \fR
\\ \verb+\Frechet+  \text{\quad---\quad}  \text{\Frechet\Frechet,text}
\\ \verb+\fhat+  \text{\quad---\quad}  \fhat
\\ \verb+\fone+  \text{\quad---\quad}  \fone
\\ \verb+\ftilde+  \text{\quad---\quad}  \ftilde
\\ \verb+\ftwo+  \text{\quad---\quad} \ftwo
\\ \verb+\ftildexialpha+  \text{\quad---\quad}  \ftildexialpha
\end{array}$


$\begin{array}{l}
  \verb+\fu+  \text{\quad---\quad}  \fu
\\ \verb+\fuplusv+  \text{\quad---\quad}   \fuplusv
\\ \verb+\fxialpha+  \text{\quad---\quad}  \fxialpha
\\ \verb+\fxialphadelta+  \text{\quad---\quad}  \fxialphadelta
\\ \verb+\fxialphahat+  \text{\quad---\quad}   \fxialphahat
\\ \verb+\fxialphan+  \text{\quad---\quad}  \fxialphan
\\ \verb+\fxialphaone+  \text{\quad---\quad}   \fxialphaone
\\ \verb+\fxialphapr+  \text{\quad---\quad}  \fxialphapr
\\ \verb+\fxialphatwo+  \text{\quad---\quad}  \fxialphatwo
\end{array}$


$\begin{array}{l}
\verb+\fxiialpha+  \text{\quad---\quad}  \fxiialpha
\\ \verb+\fxijalpha+  \text{\quad---\quad}   \fxijalpha
\\ \verb+\fxionealpha+  \text{\quad---\quad}  \fxionealpha
\\ \verb+\fxionealphahat+  \text{\quad---\quad} \fxionealphahat
\\ \verb+\fxionealphaone+  \text{\quad---\quad}  \fxionealphaone
\\ \verb+\fxionealphatwo+  \text{\quad---\quad}  \fxionealphatwo
\\ \verb+\fxipalpha+  \text{\quad---\quad}  \fxipalpha
\\ \verb+\fxipalphahat+  \text{\quad---\quad}  \fxipalphahat
\\ \verb+\fxitwoalpha+  \text{\quad---\quad}  \fxitwoalpha
\\ \verb+\fxitwoalphaone+  \text{\quad---\quad}  \fxitwoalphaone
\\ \verb+\fxitwoalphatwo+  \text{\quad---\quad} \fxitwoalphatwo
\\ \verb+\FX+  \text{\quad---\quad}  \FX
\\ \verb+\FY+  \text{\quad---\quad}  \FY
\\ \verb+\Ftilde+  \text{\quad---\quad}  \Ftilde
\end{array}$


$\begin{array}{l}
   \verb+\Galphai+  \text{\quad---\quad}  \Galphai
\\ \verb+\Galphaone+  \text{\quad---\quad}  \Galphaone
\\ \verb+\Galphatwo+  \text{\quad---\quad}  \Galphatwo
\end{array}$


$\begin{array}{l}\verb+\Gast+  \text{\quad---\quad}  \Gast
\\ \verb+\Gastone+  \text{\quad---\quad}  \Gastone
\\ \verb+\Gasttwo+  \text{\quad---\quad}  \Gasttwo
\\  \verb+\GaussDistr+  \text{\quad---\quad}  \GaussDistr
\end{array}$


$\begin{array}{l}
\verb+\Gbb+  \text{\quad---\quad}  \Gbb
\\ \verb+\GbbkPsi+  \text{\quad---\quad}  \GbbkPsi
\\ \verb+\GbbkPsiast+  \text{\quad---\quad}  \GbbkPsiast
\\ \verb+\GbbkPsiu+  \text{\quad---\quad}  \GbbkPsiu
\\ \verb+\GbbkPsik+  \text{\quad---\quad}  \GbbkPsik
\\ \verb+\GbbkPsiuk+  \text{\quad---\quad}  \GbbkPsiuk
\\ \verb+\Gbbn+  \text{\quad---\quad}  \Gbbn
\\ \verb+\GbbPsi+  \text{\quad---\quad}  \GbbPsi
\\ \verb+\GbbPsiast+  \text{\quad---\quad}  \GbbPsiast
\\ \verb+\GbbPsiu+  \text{\quad---\quad}  \GbbPsiu
\\ \verb+\Gbbtilde+  \text{\quad---\quad}  \Gbbtilde
\\ \verb+\Gbbtilden+  \text{\quad---\quad}  \Gbbtilden
\\ \verb+\GbbrhoalphaPsi+  \text{\quad---\quad}  \GbbrhoalphaPsi
\\ \verb+\Gcal+  \text{\quad---\quad}  \Gcal
\\ \verb+\GcalK+  \text{\quad---\quad}  \GcalK
\\ \verb+\galpha+  \text{\quad---\quad}  \galpha
\\ \verb+\galphadelta+  \text{\quad---\quad}  \galphadelta
\\ \verb+\galphaone+  \text{\quad---\quad}  \galphaone
\\ \verb+\galphatwo+  \text{\quad---\quad} \galphatwo
\\
  \verb+\gammaast+  \text{\quad---\quad}  \gammaast
\\ \verb+\gammaastxi+  \text{\quad---\quad}  \gammaastxi
\\ \verb+\gammaed+  \text{\quad---\quad}  \gammaed
\\ \verb+\gammaei+  \text{\quad---\quad}  \gammaei
\\ \verb+\gammaej+  \text{\quad---\quad}  \gammaej
\\ \verb+\gammaeone+  \text{\quad---\quad}  \gammaeone
\\ \verb+\gammahat+  \text{\quad---\quad}  \gammahat
\\ \verb+\gammahatxi+  \text{\quad---\quad}  \gammahatxi
\\ \verb+\gammahatxihatopt+  \text{\quad---\quad}  \gammahatxihatopt
\\ \verb+\gammaminusei+  \text{\quad---\quad}  \gammaminusei
\\ \verb+\gammaminusej+  \text{\quad---\quad}  \gammaminusej
\\ \verb+\gammaminuseone+  \text{\quad---\quad}  \gammaminuseone
\\ \verb+\gammaxi+  \text{\quad---\quad}  \gammaxi
\\ \verb+\gammaxihatopt+  \text{\quad---\quad}  \gammaxihatopt
\\ \verb+\gammaxione+  \text{\quad---\quad}  \gammaxione
\\ \verb+\gammaxiopt+  \text{\quad---\quad}  \gammaxiopt
\\ \verb+\gammaxitwo+  \text{\quad---\quad}  \gammaxitwo
\\ \verb+\Gcalalpha+  \text{\quad---\quad}  \Gcalalpha
\\ \verb+{X}\ginv+  \text{\quad---\quad}  X\ginv
\\ \verb+\grad+  \text{\quad---\quad}   \grad (= \verb+\nabla+)
\\ \verb+\gs+  \text{\quad---\quad}  \gs
\\ \verb+\gxialpha+  \text{\quad---\quad} \gxialpha
\\ \verb+\gxij+  \text{\quad---\quad}  \gxij
\\ \verb+\gxik+  \text{\quad---\quad}  \gxik
\\ \verb+\gxione+  \text{\quad---\quad}  \gxione
\end{array}$


$\begin{array}{l}
   \verb+\half+  \text{\quad---\quad}  \half
\\ \verb+\halfeps+  \text{\quad---\quad}  \halfeps
\\ \verb+\Hcal+  \text{\quad---\quad}  \Hcal
\\ \verb+\HcalH+  \text{\quad---\quad}  \HcalH
\\ \verb+\Hone+  \text{\quad---\quad}  \Hone
\\ \verb+\hu+  \text{\quad---\quad}  \hu
\\ \verb+\huv+  \text{\quad---\quad}  \huv
\\ \verb+\hxi+  \text{\quad---\quad} \hxi
\\ \verb+\hxione+  \text{\quad---\quad}  \hxione
\\ \verb+\hxitwo+  \text{\quad---\quad}  \hxitwo
\end{array}$


$\begin{array}{l}
   \verb+\Id+  \text{\quad---\quad}  Id
\\ \verb+\iid+  \text{\quad---\quad}  \iid\iid,
\\ \verb+\impl+  \text{\quad---\quad}  \impl
\\ \verb+\intzeroone+  \text{\quad---\quad}  \intzeroone
%\\ \verb+\intuzerone+  \text{\quad---\quad}  \int_{[\uzer,1]}}
%\\ \verb+\intvnone+  \text{\quad---\quad}  \int_{[\vn,1]}}
\\ \verb+\intSd+  \text{\quad---\quad}  \intSd
\\ \verb+\intSimpd+  \text{\quad---\quad}  \intSimpd
%\\ \verb+\intzerinfty+  \text{\quad---\quad}  \int_0^\infty}
%\\ \verb+\intzerovn+  \text{\quad---\quad}  \int_{[0,\vn)}}
\\ \verb+{X}\inv+  \text{\quad---\quad}  X\inv 
\end{array}$


$\begin{array}{l}
   \verb+\kappaXY+  \text{\quad---\quad}  \kappaXY
\\ \verb+\KastPsi+  \text{\quad---\quad}  \KastPsi
\\ \verb+\kn+  \text{\quad---\quad}  \kn
\\ \verb+\KPsi+  \text{\quad---\quad}  \KPsi
\end{array}$


$\begin{array}{l}\verb+\Law+  \text{\quad---\quad}  \Law
\\ \verb+\LHK+  \text{\quad---\quad}  \LHK
\end{array}$


$\begin{array}{l}\verb+\linf+  \text{\quad---\quad}  \linf
\\ \verb+\Linf+  \text{\quad---\quad}  \Linf
\\ \verb+\Lone+  \text{\quad---\quad}  \Lone
\\ \verb+\ltilde+  \text{\quad---\quad}  \ltilde
\\ \verb+\Ltwo+  \text{\quad---\quad}  \Ltwo
\end{array}$


$\begin{array}{l}\verb+\maxbin+  \text{\quad---\quad}  \maxbin
\\ \verb+\Mcal+  \text{\quad---\quad}  \Mcal
\\ \verb+\Mcalone+  \text{\quad---\quad}  \Mcalone
\\ \verb+\Mphi+  \text{\quad---\quad}  \Mphi
\\ \verb+\minbin+  \text{\quad---\quad}  \minbin
\\ \verb+\mualpha+  \text{\quad---\quad}  \mualpha
\\ \verb+\musteq+  \text{\quad---\quad}  \musteq
\\ \verb+\muPcal+  \text{\quad---\quad}  \muPcal
\\ \verb+\muX+  \text{\quad---\quad}  \muX
\\ \verb+\muY+  \text{\quad---\quad}  \muY
\\ \verb+\myalert{x}+  \text{\quad---\quad}  \myalert{xxx}
\\ \verb+\myequiv+  \text{\quad---\quad} \myequiv
\\ \verb+\myhyph+  \text{\quad---\quad}  \myhyph{}xx\myhyph zzz
\\ \verb+\mylefteqn{xxx}+  \text{\quad---\quad}  \text{Gebrauch??}
\end{array}$


$\begin{array}{l}\verb+\N+  \text{\quad---\quad}  \N
\\ \verb+\Nbr+  \text{\quad---\quad}  \Nbr
\\ \verb+X\negpart+  \text{\quad---\quad}  X\negpart
\\ \verb+\norm{\displaystyle\sum}+  \text{\quad---\quad}  \norm{\displaystyle\sum}
\\ \verb+\normfl{\displaystyle\sum}+  \text{\quad---\quad}  \normfl{\displaystyle\sum}
\\ \verb+\nstr+  \text{\quad---\quad}  \nstr
\\ \verb+\nstrstr+  \text{\quad---\quad}  \nstrstr
\\ \verb+\nualphai+  \text{\quad---\quad}  \nualphai
\\ \verb+\nuast+  \text{\quad---\quad}  \nuast
\\ \verb+\nuastone+  \text{\quad---\quad}  \nuastone
\\ \verb+\nuasttwo+  \text{\quad---\quad}  \nuasttwo
\\ \verb+\nuastX+  \text{\quad---\quad}  \nuastX
\\ \verb+\nuhat+  \text{\quad---\quad}  \nuhat
\\ \verb+\nzer+  \text{\quad---\quad}  \nzer
\end{array}$


$\begin{array}{l}
   \verb+\oneby{x}+  \text{\quad---\quad}  \oneby{x}
\\ \verb+\onebyk+  \text{\quad---\quad}  \onebyk
\\ \verb+\order+  \text{\quad---\quad}  \order
\\ \verb+\orderapl+  \text{\quad---\quad}  \orderapl
\\ \verb+\ordercx+  \text{\quad---\quad}  \ordercx
\\ \verb+\orderdcx+  \text{\quad---\quad}  \orderdcx
\end{array}$


$\begin{array}{l}
   \verb+\orderGcalalpha+  \text{\quad---\quad}  \orderGcalalpha
\\ \verb+\orderlcx+  \text{\quad---\quad}  \orderlcx
\\ \verb+\orderplcx+  \text{\quad---\quad}  \orderplcx
\\ \verb+\ordersl+  \text{\quad---\quad}  \ordersl
\\ \verb+\ordersm+  \text{\quad---\quad}  \ordersm
\\ \verb+\orderst+  \text{\quad---\quad}  \orderst
\\ \verb+\orth+  \text{\quad---\quad}   \bot
\\ \verb+x\out+  \text{\quad---\quad}  x\out
\end{array}$


$\begin{array}{l}
   \verb+\partder{x}+  \text{\quad---\quad}  \partder{x}
\\ \verb+\partderalpha+  \text{\quad---\quad}  \partderalpha
\\ \verb+\Pbb+  \text{\quad---\quad}  \Pbb
\\ \verb+\PbbkPsi+  \text{\quad---\quad}  \PbbkPsi
\\ \verb+\PbbkPsiu+  \text{\quad---\quad}  \PbbkPsiu
\\ \verb+\PbbkPsiast+  \text{\quad---\quad}  \PbbkPsiast
\\ \verb+\Pbbm+  \text{\quad---\quad}  \Pbbm
\\ \verb+\Pbbn+  \text{\quad---\quad}  \Pbbn
\\ \verb+\Pbbnstrstr+  \text{\quad---\quad}  \Pbbnstrstr
\\ \verb+\Pbbtilde+  \text{\quad---\quad}  \Pbbtilde
\\ \verb+\Pbbtilden+  \text{\quad---\quad}  \Pbbtilden
\\ \verb+\Pcal+  \text{\quad---\quad}  \Pcal
\\ \verb+\Pcalast+  \text{\quad---\quad}  \Pcalast
\\ \verb+\Pcaldiscr+  \text{\quad---\quad}  \Pcaldiscr
\\ \verb+\Pcaluzer+  \text{\quad---\quad}  \Pcaluzer
\\ \verb+\permk+  \text{\quad---\quad}  \permk
\\ \verb+\Phiast+  \text{\quad---\quad}  \Phiast
\\ \verb+\philambda+  \text{\quad---\quad}  \philambda
\\ \verb+\phizer+  \text{\quad---\quad}  \phizer
\\
   \verb+\phione+  \text{\quad---\quad}  \phione
\\ \verb+{x}\pos+  \text{\quad---\quad} x\pos
\\ \verb+{x}\pospart+  \text{\quad---\quad}  x\pospart
\\ \verb+{x}\powalpha+  \text{\quad---\quad}  x\powalpha
\\ \verb+{x}\powalphahat+  \text{\quad---\quad}  x\powalphahat
\\
   \verb+{x}\powalphaminusone+  \text{\quad---\quad}  x\powalphaminusone
\\ \verb+{x}\powalphaone+  \text{\quad---\quad}  x\powalphaone
\\ \verb+{x}\powminusalpha+  \text{\quad---\quad}  x\powminusalpha
\\ \verb+{x}\powminusonebyalpha+  \text{\quad---\quad}  x\powminusonebyalpha
\\ \verb+{x}\powonebyalpha+  \text{\quad---\quad}  x\powonebyalpha
\\
   \verb+\Prob+  \text{\quad---\quad}  \Prob
\\ \verb+\probconv+  \text{\quad---\quad}  \probconv
\\ \verb+\proboutconv+  \text{\quad---\quad}  \proboutconv
\\ \verb+\Probn+  \text{\quad---\quad}  \Probn
\\ \verb+\Probout+  \text{\quad---\quad}  \Probout
\\ \verb+\Probtilde+  \text{\quad---\quad}  \Probtilde
\\ \verb+\Probtildek+  \text{\quad---\quad}  \Probtildek
\\
   \verb+\Probtildeu+  \text{\quad---\quad}  \Probtildeu
\\ \verb+\Probtildeuk+  \text{\quad---\quad}  \Probtildeuk
\\ \verb+\ProbtildeUn+  \text{\quad---\quad}  \ProbtildeUn
\\  \verb+\ProbUn+  \text{\quad---\quad}  \ProbUn
\\ \verb+\ProbX+  \text{\quad---\quad}  \ProbX
\\ \verb+\ProbY+  \text{\quad---\quad}  \ProbY
\\
   \verb+\Psiast+  \text{\quad---\quad}  \Psiast
\\ \verb+\Psiastone+  \text{\quad---\quad}  \Psiastone
\\ \verb+\Psiasttwo+  \text{\quad---\quad}  \Psiasttwo
\\ \verb+\PsiastX+  \text{\quad---\quad}  \PsiastX
\\ \verb+\PsiastY+  \text{\quad---\quad}  \PsiastY
\\ \verb+\Psihat+  \text{\quad---\quad}  \Psihat
\end{array}$


$\begin{array}{l}
   \verb+\Psik+  \text{\quad---\quad}  \Psik
\\ \verb+\Psin+  \text{\quad---\quad}  \Psin
\\ \verb+\Psione+  \text{\quad---\quad}  \Psione
\\ \verb+\Psioneminuskbyn+  \text{\quad---\quad}  \Psioneminuskbyn
\\ \verb+\Psiprime+  \text{\quad---\quad}  \Psiprime
\\ \verb+\Psiprimeone+  \text{\quad---\quad}  \Psiprimeone
\\ \verb+\Psiprimeu+  \text{\quad---\quad}  \Psiprimeu
\\ \verb+\Psiprimeuast+  \text{\quad---\quad}  \Psiprimeuast
\\ \verb+\Psiprimev+  \text{\quad---\quad}  \Psiprimev
\\ \verb+\Psiprimezer+  \text{\quad---\quad}  \Psiprimezer
\\ \verb+\Psiu+  \text{\quad---\quad}  \Psiu
\\ \verb+\Psiuast+  \text{\quad---\quad}  \Psiuast
\\ \verb+\Psiuk+  \text{\quad---\quad}  \Psiuk
\\ \verb+\Psiun+  \text{\quad---\quad}  \Psiun
\\ \verb+\PsiUn+  \text{\quad---\quad}  \PsiUn
\\ \verb+\PsiX+  \text{\quad---\quad}  \PsiX
\\ \verb+\PsiY+  \text{\quad---\quad}  \PsiY
\end{array}$


$\begin{array}{l}\verb+\Q+  \text{\quad---\quad}  \Q
\\ \verb+\Qcal+  \text{\quad---\quad}  \Qcal
\\ \verb+\Qcalk+  \text{\quad---\quad}  \Qcalk
\\ \verb+\Qcaln+  \text{\quad---\quad}  \Qcaln
\\ \verb+\Qd+  \text{\quad---\quad}  \Qd
\end{array}$


$\begin{array}{l}
   \verb+\R+  \text{\quad---\quad}  \R
\\ \verb+\Rbar+  \text{\quad---\quad}  \Rbar
\\ \verb+\Rd+  \text{\quad---\quad}  \Rd
\\ \verb+\rhoalpha+  \text{\quad---\quad}  \rhoalpha
\\ \verb+\Rinj+  \text{\quad---\quad}  \Rinj
\\ \verb+\RinonetoRink+  \text{\quad---\quad}  \RinonetoRink
\\ \verb+\Rnkplusone+  \text{\quad---\quad}  \Rnkplusone
\\ \verb+\RnonetoRnk+  \text{\quad---\quad}  \RnonetoRnk
\end{array}$


$\begin{array}{l}
   \verb+\robr{\displaystyle\sum}+  \text{\quad---\quad}  \robr{\displaystyle\sum}
\\ \verb+\Robr{\displaystyle\sum}+  \text{\quad---\quad}  \Robr{\displaystyle\sum}
\\ \verb+\RObr{\displaystyle\sum}+  \text{\quad---\quad}  \RObr{\displaystyle\sum}
\\ \verb+\ROBr{\displaystyle\sum}+  \text{\quad---\quad}  \ROBr{\displaystyle\sum}
\\ \verb+\robrfl{\displaystyle\sum}+  \text{\quad---\quad}  \robrfl{\displaystyle\sum}
\\ \verb+\Ri+  \text{\quad---\quad}  \Ri
\\ \verb+\RonetoRn+  \text{\quad---\quad}  \RonetoRn
\\ \verb+\Rplus+  \text{\quad---\quad}  \Rplus
\\ \verb+\Rplusd+  \text{\quad---\quad}  \Rplusd
\\ \verb+\Rtilde+  \text{\quad---\quad}  \Rtilde
\\ \verb+\Rtildeinj+  \text{\quad---\quad}  \Rtildeinj
\\ \verb+\Rtildeink+  \text{\quad---\quad}  \Rtildeink
\\ \verb+\Rtildeinone+  \text{\quad---\quad}  \Rtildeinone
\\ \verb+\RX+  \text{\quad---\quad}  RX
\\ \verb+\RY+  \text{\quad---\quad}  RY
\end{array}$


$\begin{array}{l} \verb+\Sbb+  \text{\quad---\quad}  \Sbb
\\ \verb+\Scal+  \text{\quad---\quad}  \Scal
\\ \verb+\Sd+  \text{\quad---\quad}  \Sd
\\ \verb+\Sdone+  \text{\quad---\quad}  \Sdone
\\ \verb+\Sdtwo+  \text{\quad---\quad}  \Sdtwo
\\ \verb+\Sdnorm+  \text{\quad---\quad}  \Sdnorm
\\ \verb+\Sdxi+  \text{\quad---\quad}  \Sdxi
\\ \verb+\sdminusone+  \text{\quad---\quad}  \sdminusone
\\ \verb+\sdtilde+  \text{\quad---\quad}  \sdtilde
\\ \verb+x\setcomp+  \text{\quad---\quad}  x\setcomp
\\ \verb+\setcut+  \text{\quad---\quad}  \setcut
\\ \verb+\setjoin+  \text{\quad---\quad}  \setjoin (= \verb+\cup+)
\\ \verb+\setofjunctions+  \text{\quad---\quad}  \setofjunctions (= \verb+\sqcup+)
\\ \verb+\Si+  \text{\quad---\quad}  \Si
\\ \verb+\sigmaalpha+  \text{\quad---\quad}  \sigmaalpha
\\ \verb+\sigmaPsi+  \text{\quad---\quad}  \sigmaPsi
\\ \verb+\sigmaPsik+  \text{\quad---\quad}  \sigmaPsik
\\ \verb+\sign+  \text{\quad---\quad}  \sign
\\ \verb+\Sinj+  \text{\quad---\quad}  \Sinj
\\ \verb+\Simp+  \text{\quad---\quad}  \Simp (= \verb+\Sigma+)
\\ \verb+\Simpd+  \text{\quad---\quad}  \Simpd
\\ \verb+\Simpddelta+  \text{\quad---\quad}  \Simpddelta
\\ \verb+\Simptwo+  \text{\quad---\quad}  \Simptwo
\\ \verb+\Sink+  \text{\quad---\quad}  \Sink
\\ \verb+\Sinone+  \text{\quad---\quad}  \Sinone
\\ \verb+\SinonetoSink+  \text{\quad---\quad}  \SinonetoSink
\\ \verb+\sone+  \text{\quad---\quad}  \sone
\\ \verb+\sqbr{\displaystyle\sum}+ \sqbr{\displaystyle\sum}
\\ \verb+\sqbrfl{\displaystyle\sum}+ \sqbrfl{\displaystyle\sum}
\\ \verb+\sqrtk+  \text{\quad---\quad}  \sqrtk
\\ \verb+\sqrtkn+  \text{\quad---\quad}  \sqrtkn
\\ \verb+\Sr+  \text{\quad---\quad}  \Sr
\\ \verb+\Stilde+  \text{\quad---\quad}  \Stilde
\\ \verb+\Stildeinj+  \text{\quad---\quad}  \Stildeinj
\\ \verb+\Stwoone+  \text{\quad---\quad}  \Stwoone
\\ \verb+\Stwotwo+  \text{\quad---\quad}  \Stwotwo
\\ \verb+\Stwoast+  \text{\quad---\quad}  \Stwoast
\\
   \verb+\sumioned+  \text{\quad---\quad}  \sumioned
\\ \verb+\sumionek+  \text{\quad---\quad}  \sumionek
\\ \verb+\sumjonek+  \text{\quad---\quad}  \sumjonek
\end{array}$


$\begin{array}{l} \verb+\taulambda+  \text{\quad---\quad}  \taulambda
\\ \renewcommand{\theta}{\vartheta} \verb+\theta,\vartheta+  \text{\quad---\quad}  \theta \vartheta
\\ \verb+\thetaast+  \text{\quad---\quad}  \thetaast
\\ \verb+\thetahat+  \text{\quad---\quad}  \thetahat
\\ \verb+\thetahatHill+  \text{\quad---\quad}  \thetahatHill
\\ \verb+\tzer+  \text{\quad---\quad}  \tzer
\\ \verb+\toinf+  \text{\quad---\quad}  \toinf
\\ \verb+\tone+  \text{\quad---\quad}  \tone
\\ \verb+x\tr+  \text{\quad---\quad}  x\tr
\\ \verb+\tstr+  \text{\quad---\quad}  \tstr
\\ \verb+\ttwo+  \text{\quad---\quad}  \ttwo
\end{array}$


$\begin{array}{l} \verb+\uast+  \text{\quad---\quad}  \uast
\\ \verb+\Un+  \text{\quad---\quad}  \Un
\\ \verb+\UR+  \text{\quad---\quad}  \UR
\\ \verb+\un+  \text{\quad---\quad}  \un
\\ \verb+\unif+  \text{\quad---\quad}  \unif
\\ \verb+\unifDistr+  \text{\quad---\quad}  \unifDistr
\\ \verb+\uk+  \text{\quad---\quad}  \uk
\\ \verb+\uonetoud+  \text{\quad---\quad}  \uonetoud
\\ \verb+\upto+  \text{\quad---\quad}  \uparrow %alternativ \nearrow?
\\ \verb+\uzer+  \text{\quad---\quad}  \uzer
\\
\end{array}$


$\begin{array}{l} \verb+\vagueconv+  \text{\quad---\quad}  \vagueconv
\\ \verb+\Var+  \text{\quad---\quad}  \Var
\\ \verb+\VaR+  \text{\quad---\quad}  \VaR
%\\ \verb+\VaRlam+  \text{\quad---\quad}  \VaR_\lambda}
\\ \verb+\VaRoneminuslam+  \text{\quad---\quad}  \VaRoneminuslam
\\ \verb+\vn+  \text{\quad---\quad}  \vn
\\ \verb+x\vspaceone{y}+  \text{\quad---\quad} x\vspaceone{y}
\\ \verb+\vxiX+  \text{\quad---\quad}  \vxiX
\\ \verb+\vxiY+  \text{\quad---\quad}  \vxiY
\\
\end{array}$


$\begin{array}{l} \verb+\walpha+  \text{\quad---\quad}  \walpha
\\ \verb+\weakconv+  \text{\quad---\quad}  \weakconv
\\
\end{array}$


$\begin{array}{l} \verb+\Xcal+  \text{\quad---\quad}  \Xcal
%
\\ \verb+\xihat+  \text{\quad---\quad}  \xihat
\\ \verb+\xihatopt+  \text{\quad---\quad}  \xihatopt
%
% \\ \verb+\myxihat+  \text{\quad---\quad}  \widehat{\phantom{i}}\hspace{-1.15ex}\xi}
% \def\myxihat{{\mathchoice%
%   {\hspace{0.5ex}\widehat{\phantom{i}}\hspace{-1.15ex}\xi}% display mode
%   {\hspace{0.5ex}\widehat{\phantom{i}}\hspace{-1.15ex}\xi}% text mode
%   {\hspace{0.42ex}\widehat{\phantom{i}}\hspace{-0.82ex}\xi}% subscript mode
%   {\hspace{0.23ex}\widehat{\phantom{i}}\hspace{-0.73ex}\xi}% subsubscript mode
% }}
% %
% \\ \verb+\myxihatopt+  \text{\quad---\quad}  \myxihat\vphantom{\xi}opt
%
\\ \verb+\xii+  \text{\quad---\quad}  \xii
\\ \verb+\xij+  \text{\quad---\quad}  \xij
\\ \verb+\xip+  \text{\quad---\quad}  \xip
\\ \verb+\xik+  \text{\quad---\quad}  \xik
\\ \verb+\xione+  \text{\quad---\quad}  \xione
\\ \verb+\xiopt+  \text{\quad---\quad}  \xiopt
\\ \verb+\xitwo+  \text{\quad---\quad}  \xitwo
\\ \verb+\Xinj+  \text{\quad---\quad}  \Xinj
\\ \verb+\XinonetoXink+  \text{\quad---\quad}  \XinonetoXink
\\ \verb+\XonetoXn+  \text{\quad---\quad}  \XonetoXn
\\ \verb+\xonetoxn+  \text{\quad---\quad}  \xonetoxn
\\ \verb+\XonetoXd+  \text{\quad---\quad}  \XonetoXd
\\ \verb+\Xtilde+  \text{\quad---\quad}  \Xtilde
\\ \verb+\Xtildeinj+  \text{\quad---\quad}  \Xtildeinj
\\ \verb+\XtildeinonetoXtildeink+  \text{\quad---\quad}  \XtildeinonetoXtildeink\\
\end{array}$


$\begin{array}{l}
   \verb+\YinonetoYink+  \text{\quad---\quad}  \YinonetoYink
\\ \verb+\YnonetoYnk+  \text{\quad---\quad}  \YnonetoYnk
\\ \verb+\Ynkplusone+  \text{\quad---\quad}  \Ynkplusone
\\ \verb+\YonetoYd+  \text{\quad---\quad}  \YonetoYd\\
\end{array}$


$\begin{array}{l}
   \verb+\Zcal+  \text{\quad---\quad}  \Zcal
\end{array}$


\end{document}
